Dynamic Corrective Self-Distillation for Better Fine-Tuning of Pretrained Models

We tackle the challenging issue of aggressive fine-tuning encountered during the process of transfer learning of pre-trained language models (PLMs) with limited labeled downstream data. This problem primarily results in a decline in performance on the subsequent task. Inspired by the adaptive boosting method in traditional machine learning, we present an effective dynamic corrective self-distillation (DCS) approach to improve the fine-tuning of the PLMs. Our technique involves performing a self-distillation mechanism where, at each iteration, the student model actively adapts and corrects itself by dynamically adjusting the weights assigned to individual data points. This iterative self-correcting process significantly enhances the overall fine-tuning capability of PLMs, leading to improved performance and robustness. We conducted comprehensive evaluations using the GLUE benchmark demonstrating the efficacy of our method in enhancing the fine-tuning process for various PLMs across diverse downstream tasks.

==> tables/table_alpha_sensitivity.tex <==
\begin{table*}[]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccccccc|}
    \toprule
    Model/$\alpha$ & 0.1 & 0.2 & 0.3 & 0.4& 0.5 & 0.6 & 0.7 & 0.8 & 0.9 \\ \midrule
    BERT (RTE) & 67.50 & 68.59 & 71.11 & 70.39 & 71.11 & 70.03 & 70.39 & 70.38 & 68.95\\
    BERT (MRPC) & 85.04 & 84.55 & 86.76 & 86.76 & 85.78 & 86.27 & 86.04 & 86.02 & 86.25 \\
    \midrule
    RoBERTa (RTE)& 81.94 & 80.86 & 83.75 & 80.50 & 80.50 & 81.94 & 79.78 & 79.42 & 77.97 \\
    RoBERTa (MRPC)& 88.72 & 89.95 &  89.46 & 90.44 & 90.68 & 89.70 & 89.95 & 89.60 & 89.21 \\ 
    \bottomrule
    \end{tabular}}
    \caption{Sensitivity of DCS with respect to the $\alpha$ hyperparameter.}
    \label{tab:alpha}
\end{table*}

==> tables/tables_2_4_fig2.tex <==
\begin{table*}[htbp]
\centering
\begin{minipage}[b]{0.59\textwidth}
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cccc|cc}
    \toprule
    \textbf{Methods} & \textbf{CoLA} & \textbf{RTE} & \textbf{MRPC} & \textbf{STS-B} & \textbf{Avg} & $\Delta$\\
    \midrule
    Vanilla Finetuning & 63.13 & 70.18 & 90.77 & 89.61 &78.42 & 0.00 \\
    \midrule
    Weight Decay \cite{} & 63.63 &71.99 &90.93 & 89.82 & 79.09 & fff \\
    Top-K Tuning \cite{}  & 62.63 &70.90 &91.09 & 89.97 & 78.65 & fff \\
    Mixout \cite{}  & 63.60 &72.12 &91.29 & 89.99 & 79.26 & fff \\
    RecAdam \cite{}  & 64.33 &71.63 &90.85 & 89.86 & 79.17 & fff \\
    R3F*  \cite{} & 64.13 &72.28 &91.18 & 89.61 & 79.30 & fff \\
    CHILD-Tuning(F) \cite{}  & 63.71 &72.02 &91.22 & 90.18 & 79.29 & fff \\
    CHILD-Tuning(D)  & 64.92 & 73.14 &91.42 & 90.18 & 79.92 & fff \\
    \midrule
    DCS (Ours)  & 64.38 &74.36 &ccc & ddd & eee & fff \\
    \bottomrule
    \end{tabular}}
    \centering{\caption{Comparison between DCS with other existing fine-tuning methods. The values for the fine-tuning methods are taken from \cite{xu-etal-2021-raise}. Our findings show that DCS achieves similar or even best performance compared with other fine-tuning methods.}}
    \label{tab:my_dev_glue}
   \end{minipage}
   \hspace{2mm}
    \begin{minipage}[b]{0.38\textwidth}
    \centering
    \begin{minipage}[b]{\textwidth}
    \centering
    \includegraphics[width=\textwidth]{emnlp2023-latex/figures/weight_type_cropped.pdf}
    \centering{
    \captionof{figure}{Effect of different weighting strategies of DCS on the performance. Results show that leveraging the discordant teacher-student samples benefits our DCS fine-tuning framework.}}
    \label{fig:weight_strategy}       
  \end{minipage}
  \vspace{2mm}
  \end{minipage}
\end{table*}


==> tables/tables_3_4_5.tex <==
\begin{table*}[htbp]
\centering
\begin{minipage}[b]{0.48\textwidth}
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cccc|cc}
    \toprule
    \textbf{Methods} & \textbf{CoLA} & \textbf{RTE} & \textbf{MRPC} & \textbf{STS-B} & \textbf{Avg} & $\Delta$\\
    \midrule
    Vanilla Finetuning* & 63.13 & 70.18 & 90.77 & 89.61 &78.42 & 0.00 \\
    \midrule
    Weight Decay* \cite{} & 63.63 &71.99 &90.93 & 89.82 & 79.09 & fff \\
    Top-K Tuning* \cite{}  & 62.63 &70.90 &91.09 & 89.97 & 78.65 & fff \\
    Mixout* \cite{}  & 63.60 &72.12 &91.29 & 89.99 & 79.26 & fff \\
    RecAdam* \cite{}  & 64.33 &71.63 &90.85 & 89.86 & 79.17 & fff \\
    R3F*  \cite{} & 64.13 &72.28 &91.18 & 89.61 & 79.30 & fff \\
    CHILD-Tuning(F)* \cite{}  & 63.71 &72.02 &91.22 & 90.18 & 79.29 & fff \\
    CHILD-Tuning(D)*  & 64.92 & 73.14 &91.42 & 90.18 & 79.92 & fff \\
    \midrule
    DCS (Ours)  & 64.38 &74.36 &ccc & ddd & eee & fff \\
            
    \bottomrule
    \end{tabular}}
    \centering{\caption{Comparison between DCS with other existing fine-tuning methods. Results with (*) are taken from \cite{xu-etal-2021-raise}. Our findings show that DCS achieves similar or even best performance compared with other fine-tuning methods.}}
    \label{tab:my_dev_glue}
   \end{minipage}%
   \hspace{2mm}
    \begin{minipage}[b]{0.48\textwidth}
    \begin{minipage}[b]{\textwidth}
        \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccccccc|}
    \toprule
    Model/$\alpha$ & 0.1 & 0.2 & 0.3 & 0.4& 0.5 & 0.6 & 0.7 & 0.8 & 0.9 \\ \midrule
    BERT (RTE) & 67.50 & 68.59 & 71.11 & 70.39 & 71.11 & 70.03 & 70.39 & 70.38 & 68.95\\
    BERT (MRPC) & 85.04 & 84.55 & 86.76 & 86.76 & 85.78 & 86.27 & 86.04 & 86.02 & 86.25 \\
    \midrule
    RoBERTa (RTE)& 81.94 & 80.86 & 83.75 & 80.50 & 80.50 & 81.94 & 79.78 & 79.42 & 77.97 \\
    RoBERTa (MRPC)& 88.72 & 89.95 &  89.46 & 90.44 & 90.68 & 89.70 & 89.95 & 89.60 & 89.21 \\ 
    \bottomrule
    \end{tabular}}
    \caption{Sensitivity of DCS with respect to the $\alpha$ hyperparameter.}
    \label{tab:alpha}
  \end{minipage}
  \vspace{6mm}
  \begin{minipage}[b]{\textwidth}
      \centering
    \resizebox{0.5\textwidth}{6mm}{
    \begin{tabular}{l|ccccc}
    \toprule
    \textbf{Model} / \textbf{$\lambda$} & 2 & 3 & 4 & 5 & 6 \\ \midrule
    BERT-DCS  & \\
    \midrule
    RoBERTa-DCS & \\
    \bottomrule
    \end{tabular}}
    \centering{\caption{Influence of the hyper-parameter $\lambda$ on the performance of DCS.}
    \label{tab:lambda}
  \end{minipage}
        
  \end{minipage}
\end{table*}

